Design, Field Evaluation, and Traffic Analysis of a Competitive Autonomous Driving Model in a Congested Environment

Recently, numerous studies have investigated cooperative traffic systems using the communication among vehicle-to-everything (V2X). Unfortunately, when multiple autonomous vehicles are deployed while exposed to communication failure, there might be a conflict of ideal conditions between various autonomous vehicles leading to adversarial situation on the roads. In South Korea, virtual and real-world urban autonomous multi-vehicle races were held in March and November of 2021, respectively. During the competition, multiple vehicles were involved simultaneously, which required maneuvers such as overtaking low-speed vehicles, negotiating intersections, and obeying traffic laws. In this study, we introduce a fully autonomous driving software stack to deploy a competitive driving model, which enabled us to win the urban autonomous multi-vehicle races. We evaluate module-based systems such as navigation, perception, and planning in real and virtual environments. Additionally, an analysis of traffic is performed after collecting multiple vehicle position data over communication to gain additional insight into a multi-agent autonomous driving scenario. Finally, we propose a method for analyzing traffic in order to compare the spatial distribution of multiple autonomous vehicles. We study the similarity distribution between each team's driving log data to determine the impact of competitive autonomous driving on the traffic environment.

==> tables/prediction_result.tex <==
\begin{table}[hbt!]
\caption[The root mean square error (m) for each prediction time horizon and the average distance error for the Sangam dataset]{The root mean square error (m) for each prediction time horizon and the average distance error for the Sangam dataset (history 3 $s$, future 3 $s$)}
\label{sangam dataset reslut}
\centering
\begin{tabular}{c|lll}
\hline
\begin{tabular}[c]{@{}c@{}}Prediction Horizon\\ ($s$)\end{tabular} & Seq2seq~\cite{sutskever2014sequence} & GRIP++~\cite{li2020gripplus} & Proposed \\ \hline
1                                                                  & 1.7170       & 1.3115 & \textbf{1.2425}    \\
2                                                                  & 2.7965       & 2.5386 & \textbf{2.2432}   \\
3 (FDE)                                                            & 4.1398       & 2.9453 & \textbf{2.7801}    \\ \hline
ADE                                                                & 2.8844        & 2.2651  & \textbf{2.0886}    \\ \hline

\end{tabular}
\end{table}
